ECE496Y Final Report: Edge Machine Learning for Detecting Freezing of Gait in Parkinson's Patients

Parkinson's disease is a common neurological disease, entailing a multitude of motor deficiency symptoms. In this project, we developed a device with an uploaded edge machine learning algorithm that can detect the onset of freezing of gait symptoms in a Parkinson's patient. The algorithm achieved an accuracy of 83.7% in a validation using data from ten patients. The model was deployed in a microcontroller Arduino Nano 33 BLE Sense Board model and validated in real-time operation with data streamed to the microcontroller from a computer.

==> main <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{bikias2021deepfog}
T.~Bikias, D.~Iakovakis, S.~Hadjidimitriou, V.~Charisis, and L.~J.
  Hadjileontiadis, ``Deepfog: an imu-based detection of freezing of gait
  episodes in parkinson’s disease patients via deep learning,''
  \emph{Frontiers in Robotics and AI}, p. 117, 2021.

\bibitem{su2020gait}
B.~Su, C.~Smith, and E.~Gutierrez~Farewik, ``Gait phase recognition using deep
  convolutional neural network with inertial measurement units,''
  \emph{Biosensors}, vol.~10, no.~9, p. 109, 2020.

\bibitem{liu2016design}
X.~Liu, M.~Zhang, A.~G. Richardson, T.~H. Lucas, and J.~Van~der Spiegel,
  ``Design of a closed-loop, bidirectional brain machine interface system with
  energy efficient neural feature extraction and pid control,'' \emph{IEEE
  transactions on biomedical circuits and systems}, vol.~11, no.~4, pp.
  729--742, 2016.

\bibitem{bachlin2009wearable}
M.~Bachlin, M.~Plotnik, D.~Roggen, I.~Maidan, J.~M. Hausdorff, N.~Giladi, and
  G.~Troster, ``Wearable assistant for parkinson’s disease patients with the
  freezing of gait symptom,'' \emph{IEEE Transactions on Information Technology
  in Biomedicine}, vol.~14, no.~2, pp. 436--446, 2009.

\bibitem{merenda2020edge}
M.~Merenda, C.~Porcaro, and D.~Iero, ``Edge machine learning for ai-enabled iot
  devices: A review,'' \emph{Sensors}, vol.~20, no.~9, p. 2533, 2020.

\bibitem{borzi2021prediction}
L.~Borz{\`\i}, I.~Mazzetta, A.~Zampogna, A.~Suppa, G.~Olmo, and F.~Irrera,
  ``Prediction of freezing of gait in parkinson’s disease using wearables and
  machine learning,'' \emph{Sensors}, vol.~21, no.~2, p. 614, 2021.

\bibitem{liu2021edge}
X.~Liu and A.~G. Richardson, ``Edge deep learning for neural implants: a case
  study of seizure detection and prediction,'' \emph{Journal of Neural
  Engineering}, vol.~18, no.~4, p. 046034, 2021.

\bibitem{liu2021system}
------, ``A system-on-chip for closed-loop optogenetic sleep modulation,'' in
  \emph{2021 43rd Annual International Conference of the IEEE Engineering in
  Medicine \& Biology Society (EMBC)}.\hskip 1em plus 0.5em minus 0.4em\relax
  IEEE, 2021, pp. 5678--5681.

\bibitem{liu2014low}
X.~Liu, M.~Zhang, and J.~Van~der Spiegel, ``A low-power multifunctional cmos
  sensor node for an electronic fa{\c{c}}ade,'' \emph{IEEE Transactions on
  Circuits and Systems I: Regular Papers}, vol.~61, no.~9, pp. 2550--2559,
  2014.

\bibitem{brownlee2020random}
J.~Brownlee, ``Random oversampling and undersampling for imbalanced
  classification,'' \emph{Machine Learning Mastery}, 2020.

\bibitem{doshi2019various}
S.~Doshi, ``Various optimization algorithms for training neural network,''
  \emph{Towards data science}, vol.~13, 2019.

\bibitem{liu2020fully}
X.~Liu, H.~Zhu, T.~Qiu, S.~Y. Sritharan, D.~Ge, S.~Yang, M.~Zhang, A.~G.
  Richardson, T.~H. Lucas, N.~Engheta \emph{et~al.}, ``A fully integrated
  sensor-brain--machine interface system for restoring somatosensation,''
  \emph{IEEE Sensors Journal}, vol.~21, no.~4, pp. 4764--4775, 2020.

\bibitem{allibhai2018building}
E.~Allibhai, ``Building a convolutional neural network (cnn) in keras,''
  \emph{Internet draft. Towards Data Science}, 2018.

\bibitem{sharma2020keras}
P.~Sharma, ``Keras dense layer explained for beginners,'' \emph{Retrieved from
  machinelearningknowledge. ai/website: https://machinelearningknowledge.
  ai/keras-dense-layer-explained-for-beginners}, 2020.

\bibitem{liu2021energy}
X.~Liu, A.~G. Richardson, and J.~Van~der Spiegel, ``An energy-efficient
  compressed sensing-based encryption scheme for wireless neural recording,''
  \emph{IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  vol.~11, no.~2, pp. 405--414, 2021.

\bibitem{sharma2017activation}
S.~Sharma, S.~Sharma, and A.~Athaiya, ``Activation functions in neural
  networks,'' \emph{towards data science}, vol.~6, no.~12, pp. 310--316, 2017.

\bibitem{lau2019walkthrough}
S.~Lau, ``A walkthrough of convolutional neural network—hyperparameter
  tuning,'' \emph{Medium. Retrieved}, vol.~23, 2019.

\bibitem{liu2017fully}
X.~Liu, H.~Zhu, M.~Zhang, X.~Wu, A.~G. Richardson, S.~Y. Sritharan, D.~Ge,
  Y.~Shu, T.~H. Lucas, and J.~Van~der Spiegel, ``A fully integrated wireless
  sensor-brain interface system to restore finger sensation,'' in \emph{2017
  IEEE International Symposium on Circuits and Systems (ISCAS)}.\hskip 1em plus
  0.5em minus 0.4em\relax IEEE, 2017, pp. 1--4.

\bibitem{liu201512}
X.~Liu, M.~Zhang, A.~G. Richardson, T.~H. Lucas, and J.~Van~der Spiegel, ``A
  12-channel bidirectional neural interface chip with integrated channel-level
  feature extraction and pid controller for closed-loop operation,'' in
  \emph{2015 IEEE Biomedical Circuits and Systems Conference (BioCAS)}.\hskip
  1em plus 0.5em minus 0.4em\relax IEEE, 2015, pp. 1--4.

\bibitem{liu2013low}
X.~Liu, M.~Zhang, and J.~Van~der Spiegel, ``A low power multi-mode cmos image
  sensor with integrated on-chip motion detection,'' in \emph{2013 IEEE
  international symposium on circuits and systems (ISCAS)}.\hskip 1em plus
  0.5em minus 0.4em\relax IEEE, 2013, pp. 2416--2419.

\end{thebibliography}

